The Incredible Shrinking Context... in a Decompiler Near You

Decompilation of binary code has arisen as a highly-important application in the space of Ethereum VM (EVM) smart contracts. Major new decompilers appear nearly every year and attain popularity, for a multitude of reverse-engineering or tool-building purposes. Technically, the problem is fundamental: it consists of recovering high-level control flow from a highly-optimized continuation-passing-style (CPS) representation. Architecturally, decompilers can be built using either static analysis or symbolic execution techniques. We present Shrknr, a static-analysis-based decompiler succeeding the state-of-the-art Elipmoc decompiler. Shrknr manages to achieve drastic improvements relative to the state of the art, in all significant dimensions: scalability, completeness, precision. Chief among the techniques employed is a new variant of static analysis context: shrinking context sensitivity. Shrinking context sensitivity performs deep cuts in the static analysis context, eagerly "forgetting" control-flow history, in order to leave room for further precise reasoning. We compare Shrnkr to state-of-the-art decompilers, both static-analysis- and symbolic-execution-based. In a standard benchmark set, Shrnkr scales to over 99.5% of contracts (compared to ~95%), covers (i.e., reaches and manages to decompile) 67% more code, and reduces key imprecision metrics by over 65%.

==> experiments/workspace/heimdal/signature-dominance-sigs-eli.tex <==
\begin{tabular}{|c|c|c|}
    \toprule
    {}           &  External Calls   &  Events  \\
    \midrule
    \#Instances of \ourtool{} dominance instances  &                    1590\textbf{(\textasciitilde{}32\%)} &         1338\textbf{(\textasciitilde{}27\%)}   \\
    \#Instances of \heimdall{} dominance instances &                     202\textbf{(\textasciitilde{}4\%)} &           5\textbf{(\textasciitilde{}0\%)}  \\
    Largest \ourtool{} dominance diff  &                    38 &         19   \\
    Largest \heimdall{} dominance diff  &                    5 &         14   \\
    \#Instances with commonly 0 identified signatures &                    2350\textbf{(\textasciitilde{}47\%)} &         1886\textbf{(\textasciitilde{}38\%)}   \\
    \#Instances with equal (non-zero) \#identified signatures &                    845\textbf{(\textasciitilde{}17\%)} &         1758\textbf{(\textasciitilde{}35\%)}   \\

    \bottomrule
\end{tabular}
    

==> experiments/workspace/heimdal/signature-dominance-sigs-viair.tex <==
\begin{tabular}{|c|c|c|}
    \toprule
    {}           &  External Calls   &  Events  \\
    \midrule
    \#Instances of \ourtool{} dominance  &                    1384\textbf{(\textasciitilde48\%)} &         1413\textbf{(\textasciitilde49\%)}   \\
    \#Instances of \heimdall{} dominance  &                     192\textbf{(\textasciitilde6\%)} &           43\textbf{(\textasciitilde1\%)}  \\
    Largest \ourtool{} dominance diff  &                    27 &         22   \\
    Largest \heimdall{} dominance diff  &                    18 &         2   \\
    \#Instances with commonly 0 identified signatures &                    525\textbf{(\textasciitilde18\%)} &         665\textbf{(\textasciitilde23\%)}   \\
    \#Instances with equal (non-zero) \#identified signatures &                    805\textbf{(\textasciitilde28\%)} &         785\textbf{(\textasciitilde27\%)}   \\


    \bottomrule
\end{tabular}
    

==> experiments/workspace/standard-dataset/shrinker-design-decisions-metrics.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
\toprule
{} &  Polymorphic Jump Target &  Missing Control Flow &  Missing TAC Block &  Unresolved Operand &  Unstructured Control Flow \\
\midrule
No Shrinking ctx &                     3406 &                   459 &                751 &                 128 &                        611 \\
No Cloning       &                       18 &                   728 &                153 &                 140 &                       1042 \\
No Incomplete    &                       40 &                   421 &                  3 &                  62 &                        542 \\
Shrnkr           &                       19 &                   421 &                  3 &                  62 &                        542 \\
\bottomrule
\end{tabular}


==> experiments/workspace/standard-dataset/shrinker-design-decisions-timeouts.tex <==
\begin{tabular}{|c|c|c|}
\toprule
{} &  Timeout \\
\midrule
No Shrinking ctx &      559 \\
No Cloning       &       16 \\
No Incomplete    &       19 \\
Shrnkr           &       13 \\
\bottomrule
\end{tabular}


==> experiments/workspace/standard-dataset/shrinker-elipmoc-metrics.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
\toprule
{} &  Polymorphic Jump Target &  Missing Control Flow &  Missing TAC Block &  Unresolved Operand &  Unstructured Control Flow \\
\midrule
Elipmoc &                     4118 &                  9411 &               1712 &                 202 &                       2253 \\
Shrnkr  &                       19 &                   424 &                  3 &                 108 &                        667 \\
\bottomrule
\end{tabular}


==> experiments/workspace/standard-dataset/shrinker-elipmoc-timeouts.tex <==
\begin{tabular}{|c|c|c|}
\toprule
{} &  Timeout \\
\midrule
Elipmoc &      235 \\
Shrnkr  &       13 \\
\bottomrule
\end{tabular}


==> experiments/workspace/yul-dataset/shrinker-design-decisions-metrics.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
\toprule
{} &  Polymorphic Jump Target &  Missing Control Flow &  Missing TAC Block &  Unresolved Operand &  Unstructured Control Flow \\
\midrule
No Shrinking ctx &                     3381 &                   253 &               1474 &                 333 &                       3624 \\
No Cloning       &                       34 &                   168 &               1602 &                 504 &                       6568 \\
No Incomplete    &                      101 &                   121 &                956 &                 184 &                       2927 \\
Shrnkr           &                       65 &                   120 &                956 &                 184 &                       2927 \\
\bottomrule
\end{tabular}


==> experiments/workspace/yul-dataset/shrinker-design-decisions-timeouts.tex <==
\begin{tabular}{|c|c|c|}
\toprule
{} &  Timeout \\
\midrule
No Shrinking ctx &      403 \\
No Cloning       &      105 \\
No Incomplete    &      146 \\
Shrnkr           &       94 \\
\bottomrule
\end{tabular}


==> experiments/workspace/yul-dataset/shrinker-elipmoc-metrics.tex <==
\begin{tabular}{|c|c|c|c|c|c|}
\toprule
{} &  Polymorphic Jump Target &  Missing Control Flow &  Missing TAC Block &  Unresolved Operand &  Unstructured Control Flow \\
\midrule
Elipmoc &                     2288 &                  1221 &               2443 &                2116 &                       7410 \\
Shrnkr  &                       74 &                   145 &               1161 &                 196 &                       3057 \\
\bottomrule
\end{tabular}


==> experiments/workspace/yul-dataset/shrinker-elipmoc-timeouts.tex <==
\begin{tabular}{|c|c|c|}
\toprule
{} &  Timeout \\
\midrule
Elipmoc &      379 \\
Shrnkr  &       94 \\
\bottomrule
\end{tabular}

